DiVinE-CUDA - A Tool for GPU Accelerated LTL Model Checking

In this paper we present a tool that performs CUDA accelerated LTL Model Checking. The tool exploits parallel algorithm MAP adjusted to the NVIDIA CUDA architecture in order to efficiently detect the presence of accepting cycles in a directed graph. Accepting cycle detection is the core algorithmic procedure in automata-based LTL Model Checking. We demonstrate that the tool outperforms non-accelerated version of the algorithm and we discuss where the limits of the tool are and what we intend to do in the future to avoid them.

==> eptcsdata.tex <==
\providecommand{\event}{L. Brim and J. van de Pol (Eds.): 8th International Workshop\\
on Parallel and Distributed Methods in verifiCation 2009 (PDMC'09)}
\providecommand{\volume}{14}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{107}
\providecommand{\eid}{8}
\pdfoutput=1

